Ergodic Capacity of Discrete- and Continuous-Time, Frequency-Selective Rayleigh Fading Channels with Correlated Scattering

We study the ergodic capacity of a frequency-selective Rayleigh fading channel with correlated scattering, which finds application in the area of UWB. Under an average power constraint, we consider a single-user, single-antenna transmission. Coherent reception is assumed with full CSI at the receiver and no CSI at the transmitter. We distinguish between a continuous- and a discrete-time channel, modeled either as random process or random vector with generic covariance. As a practically relevant example, we examine an exponentially attenuated Ornstein-Uhlenbeck process in detail. Finally, we give numerical results, discuss the relation between the continuous- and the discrete-time channel model and show the significant impact of correlated scattering.

==> lib/layout_lib.tex <==
%##############################################################################
%
% Description: This file includes settings for a common layout.
%
% Copyright (C) 2002 Christian Müller
%
%   $Author: muellerc $
%     $Date: 2005/09/19 12:21:56 $
%  $RCSfile: layout_lib.tex,v $
% $Revision: 1.1 $
%     $Name:  $
%
% This program is free software; you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation; either version 2, or (at your option)
% any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
%
% You should have received a copy of the GNU General Public License
% along with this program; if not, write to the Free Software
% Foundation, Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%
% Have a lot of fun ...
%
%##############################################################################


%##############################################################################
% USED PACKAGES
%##############################################################################

%* provides the \ifthenelse and \whiledo commands *****************************
\usepackage{ifthen}

%* provides the right, case depending white spaces within new commands ********
\usepackage{xspace}

%* provides colored text and background ***************************************
\usepackage{color}

%* provides extended array functionality **************************************
\usepackage{array}

%* provides tables of a given width *******************************************
\usepackage{tabularx}

%* provides extended verbatim environment *************************************
\usepackage{verbatim}


%##############################################################################
% MAKES SURE THIS FILE WILL BE PUT IN ONLY ONCE
%##############################################################################

%******************************************************************************
% Please don't remove the following lines to be sure  new  definitions in  this
% file will only be made once (they work like the  "#ifndef.. #define.. #endif"
% commands in headers for  C  or  C++  sources).  If you remove them you'll get
% error messages for nested inputs. Ok, how dose it work:
%
% 1st line:      if (\<name of file> is not defined) then 
%                   define \<name of file> to be the string "new defined"
%                else
%                   leave the the command \<name of file> untouched
%
% from 2nd line: if (\<name of file> == "new defined") then
%                   redefine \<name of file> to be the string "redefined"
%                   .
%                   input everything from this into the calling file
%                   .
%                else
%                   don't do anything
%
% P.S. Just to remind you,  names for new commands may only include characters.
%      This  file  for  example  has  the  name  "layout_library.tex"  and  the
%      corresponding command got the name  "\LayoutLibrary".
%
%******************************************************************************
\providecommand*{\LayoutLib}{new defined}
\ifthenelse{\equal{\LayoutLib}{new defined}}{
\renewcommand*{\LayoutLib}{redefined}


%##############################################################################
% INCLUDES OR INPUTS
%##############################################################################


%##############################################################################
% DEFINES
%##############################################################################


%##############################################################################
% NEW LENGTHS
%##############################################################################


%##############################################################################
% NEW COMMANDS
%##############################################################################

%* emphasize environment that ensures space behind ****************************
\newcommand{\Xemph}[1]{\emph{#1}\xspace}

%* text environment in small caps that ensures space behind *******************
\newcommand{\Xsc}[1]{{\sc{#1}}\xspace}

%* text environment that ensures space behind *********************************
\newcommand{\Xtext}[1]{\ensuremath{\text{#1}}\xspace}

%* provides common format of value with unit **********************************
\newcommand{\Value}[2]{\mbox{\ensuremath{#1}\,#2}}


%##############################################################################
% NEW COLUMN TYPES
%##############################################################################

%* table header required for column typs with other fonts and/or size *********
\newcommand{\TableHead}[1]{\normalfont\normalsize{#1}}

%* mathematical column type where #1 is in {l, c, r} **************(array.sty)*
\newcolumntype{M}[1]{>{$}#1<{$}}

%* typewriter column type *****************************************(array.sty)*
\newcolumntype{T}{>{\small\tt}l}

%* explanation column type *************************************(tabularx.sty)*
\newcolumntype{E}{>{\small}X}


%##############################################################################
% NEW COLUMN TYPES
%##############################################################################

\newcommand{\multirow}[2]{\raisebox{#1}[-#1]{#2}}


%##############################################################################
% NEW COLORS
%##############################################################################

%* light gray (requires color.sty) ********************************************
\definecolor{LightGray}{gray}{0.9}


%##############################################################################
% END OF FILE
%##############################################################################

}{} %* \ifthenelse at the beginning of this file (don't remove the brackets) **

%******************************************************************************
%
% $Log: layout_lib.tex,v $
% Revision 1.1  2005/09/19 12:21:56  muellerc
% - moved templates into documents subfolder
%
% Revision 1.1  2005/09/14 16:03:17  muellerc
% - added template for writing a paper
%
% Revision 1.2  2005/09/06 12:58:02  muellerc
% - removed input of math_lib.tex
%
% Revision 1.1  2005/09/05 16:09:50  muellerc
% - added template for minutes of meeting
%
%******************************************************************************


==> lib/names_lib.tex <==
%##############################################################################
%
% Description: LaTeX library including names of famous persons.
%
% Copyright (C) 2002 Christian Müller
%
%   $Author: muellerc $
%     $Date: 2005/09/19 12:21:56 $
%  $RCSfile: names_lib.tex,v $
% $Revision: 1.1 $
%     $Name:  $
%
% This program is free software; you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation; either version 2, or (at your option)
% any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
%
% You should have received a copy of the GNU General Public License
% along with this program; if not, write to the Free Software
% Foundation, Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%
% Have a lot of fun ...
%
%##############################################################################

%##############################################################################
% USED PACKAGES
%##############################################################################

%* provides the \ifthenelse and \whiledo commands *****************************
\usepackage{ifthen}


%##############################################################################
% MAKES SURE THIS FILE WILL BE INPUT ONLY ONCE
%##############################################################################

%******************************************************************************
% Please don't remove the following lines to be sure  new  definitions in  this
% file will only be made once (they work like the  "#ifndef.. #define.. #endif"
% commands in headers for  C  or  C++  sources).  If you remove them you'll get
% error messages for nested inputs. Ok, how dose it work:
%
% 1st line:      if (\<name of file> is not defined) then 
%                   define \<name of file> to be the string "new defined"
%                else
%                   leave the the command \<name of file> untouched
%
% from 2nd line: if (\<name of file> == "new defined") then
%                   redefine \<name of file> to be the string "redefined"
%                   .
%                   input everything from this into the calling file
%                   .
%                else
%                   don't do anything
%
% P.S. Just to remind you,  names for new commands may only include characters.
%      This  file  for  example  has  the  name  "template-input.tex"  and  the
%      corresponding command got the name  "\TemplateInput".
%
%******************************************************************************
\providecommand*{\NamesLib}{new defined}
\ifthenelse{\equal{\NamesLib}{new defined}}{
\renewcommand*{\NamesLib}{redefined}


%##############################################################################
% INCLUDES OR INPUTS
%##############################################################################


%##############################################################################
% DEFINES
%##############################################################################


%##############################################################################
% LENGTHS, NEW OR CHANGED
%##############################################################################


%##############################################################################
% COMMANDS, NEW OR CHANGED
%##############################################################################

\newcommand{\Banach}{\Xsc{Banach}}

\newcommand{\Bernoulli}{\Xsc{Bernoulli}}

\newcommand{\Boltzmann}{\Xsc{Boltzmann}}

\newcommand{\Borel}{\Xsc{Borel}}

\newcommand{\Cauchy}{\Xsc{Cauchy}}

\newcommand{\Cramer}{\Xsc{Cramer}}

\newcommand{\Dirac}{\Xsc{Dirac}}

\newcommand{\Euler}{\Xsc{Euler}}

\newcommand{\Fatou}{\Xsc{Fatou}}

\newcommand{\Fourier}{\Xsc{Fourier}}

\newcommand{\Gateaux}{\Xsc{G\^{a}teaux}}

\newcommand{\Gauss}{\Xsc{Gauss}}

\newcommand{\Gronwall}{\Xsc{Gronwall}}

\newcommand{\Hamilton}{\Xsc{Hamilton}}

\newcommand{\Hesse}{\Xsc{Hesse}}

\newcommand{\Hospital}{\Xsc{de l'Hospital}}

\newcommand{\Jacobi}{\Xsc{Jacobi}}

\newcommand{\Jensen}{\Xsc{Jensen}}

\newcommand{\Lagrange}{\Xsc{Lagrange}}

\newcommand{\Laplace}{\Xsc{Laplace}}

\newcommand{\Leibniz}{\Xsc{Leibniz}}

\newcommand{\Legendre}{\Xsc{Legendre}}

\newcommand{\Lindeloef}{\Xsc{Lindelöf}}

\newcommand{\Lionville}{\Xsc{Lionville}}

\newcommand{\Lipschitz}{\Xsc{Lipschitz}}

\newcommand{\Newton}{\Xsc{Newton}}

\newcommand{\Nikodym}{\Xsc{Nikodym}}

\newcommand{\Picard}{\Xsc{Picard}}

\newcommand{\Radon}{\Xsc{Radon}}

\newcommand{\Steinitz}{\Xsc{Steinitz}}

\newcommand{\Sturm}{\Xsc{Sturm}}

\newcommand{\Taylor}{\Xsc{Taylor}}

\newcommand{\Wronski}{\Xsc{Wronski}}

\newcommand{\Zorn}{\Xsc{Zorn}}


%##############################################################################
% END OF FILE
%##############################################################################

}{} %* \ifthenelse at the beginning of this file (don't remove the brackets) **

%******************************************************************************
%
% $Log: names_lib.tex,v $
% Revision 1.1  2005/09/19 12:21:56  muellerc
% - moved templates into documents subfolder
%
% Revision 1.1  2005/09/14 16:03:17  muellerc
% - added template for writing a paper
%
% Revision 1.1  2005/09/05 16:09:50  muellerc
% - added template for minutes of meeting
%
%******************************************************************************

